Kollaps: Decentralized and Dynamic Topology Emulation

The performance and behavior of large-scale distributed applications is highly influenced by network properties such as latency, bandwidth, packet loss, and jitter. For instance, an engineer might need to answer questions such as: What is the impact of an increase in network latency in application response time? How does moving a cluster between geographical regions affect application throughput? How network dynamics affects application stability? Answering these questions in a systematic and reproducible way is very hard, given the variability and lack of control over the underlying network. Unfortunately, state-of-the-art network emulation or testbeds scale poorly (i.e., MiniNet), focus exclusively on the control-plane (i.e., CrystalNet) or ignore network dynamics (i.e., EmuLab). Kollaps is a fully distributed network emulator that address these limitations. Kollaps hinges on two key observations. First, from an application's perspective, what matters are the emergent end-to-end properties (e.g., latency, bandwidth, packet loss, and jitter) rather than the internal state of the routers and switches leading to those properties. This premise allows us to build a simpler, dynamically adaptable, emulation model that circumvent maintaining the full network state. Second, this simplified model is maintainable in a fully decentralized way, allowing the emulation to scale with the number of machines for the application. Kollaps is fully decentralized, agnostic of the application language and transport protocol, scales to thousands of processes and is accurate when compared against a bare-metal deployment or state-of-the-art approaches that emulate the full state of the network. We showcase how Kollaps can accurately reproduce results from the literature and predict the behaviour of a complex unmodified distributed key-value store (i.e., Cassandra) under different deployments.

==> annexes.tex <==
\section{TC abstraction layer API}
\label{sec:tcAPI}
The tc abstraction layer exposes the API given Listing~\ref{TCAL_API}.
\\
\begin{minipage}{\linewidth}
\begin{lstlisting}[style=cpp, caption={tc abstraction layer API}, label=TCAL_API]
void init(short controlPort);
void initDestination(
        std::string ip, int bandwidth, 
        int latency, float jitter, 
        float packetLoss);
void changeBandwidth(
        std::string ip, 
        int bandwidth);
void updateUsage();
unsigned long queryUsage(std::string ip);
void tearDown();
\end{lstlisting}
\end{minipage}

The {\texttt init} function initializes the tc infrastructure.
It receives as argument a port address for the control port, used to exchange metadata and commands between emulation core instances.
The {\texttt initDestination} function sets up the tc infrastructure for enforcing delay, packet loss and bandwidth throttling on all traffic directed to the specified IP address.
The {\texttt changeBandwidth} function modifies the tc infrastructure changing the maximum allowed bandwidth to the specified IP address.
The {\texttt updateUsage} function takes a snapshot of the number of bytes sent to each previously setup destination.
The {\texttt queryUsage} function retrieves this information for a specific destination.
The {\texttt tearDown} function destroys all the created tc infrastructure.


==> workflow.tex <==
\section{Workflow}
\label{sec:workflow}
In this section we describe the workflow when using \sys.
%\mm{Paulo, update this to match the current implementation, namely the extension of the images} 
%\pg{the workflow is still the same, the difference in the extension of the images is that there is no longer NEED inside other containers, it is all injected from the god container.}
%Figure~\ref{img:workflow}\mm{TODO} depicts the workflow required to set up an experiment with \sys.
We assume the existence of a working Docker Swarm~\cite{dockerswarm} or Kubernetes~\cite{k8s} environment.

%\begin{figure}
%\centering
%\includegraphics[scale=0.4]{images/architectureV3.pdf}
%\caption{\sys{} workflow.\mm{TODO: placeholder. Remove swarm and EC stuff.}}
%\label{img:workflow}
%\end{figure}
%
Given an existing container image, the user extends it using a provided \sys template to produce a new image.
Listing~\ref{lst:cassandra} shows how we extended an third-party Cassandra Docker image for our Cassandra experiments in Section~\ref{sec:evaluation}. 

\begin{figure}
%\begin{minipage}{\linewidth}
\begin{lstlisting}[style=dockerfile, basicstyle=\footnotesize, caption={Example of extending a third-party Docker image of the Cassandra NoSQL datastore to be used with \textsc{Need}.},captionpos=b, label=lst:cassandra]
FROM cassandra:3.11
ADD ./need-entrypoint.sh /
ENTRYPOINT ["/bin/sh", "/need-entrypoint.sh"]
\end{lstlisting}
\end{figure}

Then, the user defines a topology description given as input to the deployment generator.
The Deployment Generator produces a new container composition description (a Docker Compose File~\cite{dockercompose} in the current prototype) which will be used by the underlying container orchestration framework (currently Docker Swarm~\cite{dockerswarm}).
Once deployed over the cluster (deploy step), the Emulation Manager (Section~\ref{sec:emuCore}) executes inside each container alongside the application code and takes care of enforcing the characteristics of the topology.

This entails setting up the initial network conditions, monitoring and shaping outbound traffic to match current application traffic within the constraints of the topology, as well as communicating with other core instances to maintain the state of the topology.

